Neural Compress-and-Forward for the Primitive Diamond Relay Channel

The diamond relay channel, where a source communicates with a destination via two parallel relays, is one of the canonical models for cooperative communications. We focus on the primitive variant, where each relay observes a noisy version of the source signal and forwards a compressed description over an orthogonal, noiseless, finite-rate link to the destination. Compress-and-forward (CF) is particularly effective in this setting, especially under oblivious relaying where relays lack access to the source codebook. While neural CF methods have been studied in single-relay channels, extending them to the two-relay case is non-trivial, as it requires fully distributed compression without any inter-relay coordination. We demonstrate that learning-based quantizers at the relays can harness input correlations by operating remote, yet in a collaborative fashion, enabling effective distributed compression in line with Berger-Tung-style coding. Each relay separately compresses its observation using a one-shot learned quantizer, and the destination jointly decodes the source message. Simulation results show that the proposed scheme, trained end-to-end with finite-order modulation, operates close to the known theoretical bounds. These results demonstrate that neural CF can scale to multi-relay systems while maintaining both performance and interpretability.

==> Diamond_neural_CF-2/common.tex <==
\usepackage{amsmath,amssymb,amsfonts,bbm,bm,mathrsfs}
\usepackage{color}
\usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{xcolor}
% \usepackage{hyperref}
\usepackage{amsthm}

% \usepackage{flushend}

\usepackage[ruled,vlined,linesnumbered]{algorithm2e}

\usepackage[mode=tex]{standalone} % mode=image|tex, mode=build, buildmissing


\usepackage{tikz}
% \usepackage{tkz-graph}

\usepackage{chronosys}
\usepackage{xspace}
\usetikzlibrary{shapes,arrows,calc,positioning,fit,automata}
\usetikzlibrary{decorations.markings}
\usetikzlibrary{overlay-beamer-styles}
\usepackage{fontawesome}

\usepackage{pgfplots}
\usepackage{pgfplotstable}
\usepackage{filecontents}

\usepackage{caption,subcaption}

\usepackage{soul}


==> Diamond_neural_CF-2/conference_paper/Sections/2_system_model.tex <==
\begin{figure}
    \centering
    \includestandalone[width=1\columnwidth]{fig_data/diamond_cf_diagram}
    \vspace{-1.5em}
    \caption{Diagram
    }
    \label{fig:rate_vs_overall_performance}
\end{figure}

==> Diamond_neural_CF-2/conference_paper/Sections/5_simulation_results.tex <==
\begin{comment}
\begin{figure}
    \centering
    \includestandalone[width=1\columnwidth]{fig_data/real_marginal/real_marginal_curve}
    \vspace{-1.5em}
    \caption{Caption
    }
    \label{fig:4pam}
\end{figure}

\begin{figure}
    \centering
    \includestandalone[width=1\columnwidth]{fig_data/complex_marginal/complex_marginal_curve}
    \vspace{-1.5em}
    \caption{Caption
    }
    \label{fig:4qam}
\end{figure}
\end{comment}

\begin{figure}
    \centering
     \includegraphics[width=\linewidth]{Images/4pam_marginal_visualization_with_encoder.pdf}
    \vspace{-1.5em}
    \caption{Caption
    }
    \label{fig:4qam}
\end{figure}

\begin{figure}
    \centering
    \includestandalone[width=1\columnwidth]{fig_data/multistep/ser_curve}
    \includestandalone[width=1\columnwidth]{fig_data/multistep/capacity_curve}
    \vspace{-1.5em}
    \caption{SER and mutual information
    }
    \label{fig:rate_vs_overall_performance}
\end{figure}


\begin{figure}
    \centering
     \includegraphics[width=\linewidth]{Images/4pam_multistep_visualization.pdf}
    \vspace{-1.5em}
    \caption{Caption
    }
    \label{fig:4qam}
\end{figure}

\begin{figure*}[htbp]
    \centering
    \begin{minipage}{0.49\textwidth}
        \centering
        \includestandalone[width=1\columnwidth]{fig_data/real_marginal/real_marginal_curve}
        \caption{First figure caption.}
        \label{fig:fig1}
    \end{minipage}
    \hfill
    \begin{minipage}{0.49\textwidth}
        \centering
        \includestandalone[width=1\columnwidth]{fig_data/complex_marginal/complex_marginal_curve}
        \caption{Second figure caption.}
        \label{fig:fig2}
    \end{minipage}
\end{figure*}

==> conference_paper/Sections/2_system_model.tex <==
\begin{figure}
    \centering
    \includestandalone[width=1\columnwidth]{fig_data/diamond_cf_diagram}
    \vspace{-1.5em}
    \caption{Diagram
    }
    \label{fig:rate_vs_overall_performance}
\end{figure}

==> conference_paper/Sections/5_simulation_results.tex <==
\begin{comment}
\begin{figure}
    \centering
    \includestandalone[width=1\columnwidth]{fig_data/real_marginal/real_marginal_curve}
    \vspace{-1.5em}
    \caption{Caption
    }
    \label{fig:4pam}
\end{figure}

\begin{figure}
    \centering
    \includestandalone[width=1\columnwidth]{fig_data/complex_marginal/complex_marginal_curve}
    \vspace{-1.5em}
    \caption{Caption
    }
    \label{fig:4qam}
\end{figure}
\end{comment}

\begin{figure}
    \centering
     \includegraphics[width=\linewidth]{Images/4pam_marginal_visualization_with_encoder.pdf}
    \vspace{-1.5em}
    \caption{Caption
    }
    \label{fig:4qam}
\end{figure}

\begin{figure}
    \centering
    \includestandalone[width=1\columnwidth]{fig_data/multistep/ser_curve}
    \includestandalone[width=1\columnwidth]{fig_data/multistep/capacity_curve}
    \vspace{-1.5em}
    \caption{SER and mutual information
    }
    \label{fig:rate_vs_overall_performance}
\end{figure}


\begin{figure}
    \centering
     \includegraphics[width=\linewidth]{Images/4pam_multistep_visualization.pdf}
    \vspace{-1.5em}
    \caption{Caption
    }
    \label{fig:4qam}
\end{figure}

\begin{figure*}[htbp]
    \centering
    \begin{minipage}{0.49\textwidth}
        \centering
        \includestandalone[width=1\columnwidth]{fig_data/real_marginal/real_marginal_curve}
        \caption{First figure caption.}
        \label{fig:fig1}
    \end{minipage}
    \hfill
    \begin{minipage}{0.49\textwidth}
        \centering
        \includestandalone[width=1\columnwidth]{fig_data/complex_marginal/complex_marginal_curve}
        \caption{Second figure caption.}
        \label{fig:fig2}
    \end{minipage}
\end{figure*}
